Reducing the Depth of Quantum FLT-Based Inversion Circuit

Works on quantum computing and cryptanalysis has increased significantly in the past few years. Various constructions of quantum arithmetic circuits, as one of the essential components in the field, has also been proposed. However, there has only been a few studies on finite field inversion despite its essential use in realizing quantum algorithms, such as in Shor's algorithm for Elliptic Curve Discrete Logarith Problem (ECDLP). In this study, we propose to reduce the depth of the existing quantum Fermat's Little Theorem (FLT)-based inversion circuit for binary finite field. In particular, we propose follow a complete waterfall approach to translate the Itoh-Tsujii's variant of FLT to the corresponding quantum circuit and remove the inverse squaring operations employed in the previous work by Banegas et al., lowering the number of CNOT gates (CNOT count), which contributes to reduced overall depth and gate count. Furthermore, compare the cost by firstly constructing our method and previous work's in Qiskit quantum computer simulator and perform the resource analysis. Our approach can serve as an alternative for a time-efficient implementation.

==> kotretan.tex <==
PENTING:
mau bahasanya: sequential arrangemen of values, atau waterfall approach... dkkk bebas


https://docs.google.com/document/d/1AKFF911mUyglX0YcUjLiETJy7Vztarzr0rMRAlRSpsc/edit


content:
- recent advances in qc has shown promising result in .....significant advantages in ...
- particularly, since shor's algorithm: quantum cryptanalysis
- in the near future, an ideal, noiseless qc era has not yet to be seen, but many initiatives has geared towards quantum advantages for NISQ era.
Nvertheless, sooner or later, 
- later, naik juga technological advances in no of qubits dkk, quantum operations become as important.


In the quantum case itself, constructing a quantum circuit has been a challenge due to constraints......


In quantum, some considerations need to be taken into account: depth, width, size...

Mostly on T-depth
but more and more (?) argue that in the end we will need to take into account overall metrics rather than specifically suppress the T-depth. 

/ we need to start considering the overall metric / other metrics...

As 

In this paper, we provide alternative that reduces the number of T-depth 



Classically, there are two types of algorithm commonly used to perform inversion, namely the Extended Euclidean Algorithm (EEA) and Fermat's Little Theorem (FLT) \cite{NadikudaClassicalInversion}. As for the latter, the most frequently used is the variant proposed by Itoh-Tsujii, which basically performs the exponentiation via "smart" repeated squaring to give lower number of multiplications. 

Fig.
Table

(1) --> use Equation only at the first word in sentence
lol \cite{NadikudaClassicalInversion}

contribution

% organization 
\hl{BIKIN COVER LETTER, jelaskan why you want to submit to ieee access rather than TQE, and that's why we give elaborate description in the preliminaries!}
